Abstractors and relational cross-attention: An inductive bias for explicit relational reasoning in Transformers

An extension of Transformers is proposed that enables explicit relational reasoning through a novel module called the Abstractor. At the core of the Abstractor is a variant of attention called relational cross-attention. The approach is motivated by an architectural inductive bias for relational learning that disentangles relational information from object-level features. This enables explicit relational reasoning, supporting abstraction and generalization from limited data. The Abstractor is first evaluated on simple discriminative relational tasks and compared to existing relational architectures. Next, the Abstractor is evaluated on purely relational sequence-to-sequence tasks, where dramatic improvements are seen in sample efficiency compared to standard Transformers. Finally, Abstractors are evaluated on a collection of tasks based on mathematical problem solving, where consistent improvements in performance and sample efficiency are observed.

==> experiments_discriminative_longer.tex <==
\subsection{Discriminative relational tasks}\label{ssec:experiments_discriminative}
\subsubsection{Order relations: modeling asymmetric relations}\label{sssec:exp_order_relation}
A recent closely related work is~\citep{kerg2022neural}, which identifies and argues for certain inductive biases in relational models. They propose a model called CoRelNet which is, in some sense, the simplest possible model which satisfies those inductive biases. They show that this model is capable of outperforming several previous explicitly relation architectures. One inductive bias which they argue for is to model relations between objects as \textit{symmetric} inner products between object representations. %In this section, we aim to add to the discussion on inductive biases for relational learning by arguing that a general relational architecture needs to be able to model asymmetric relations as well.

The CoRelNet architecture is as follows: given a sequence of objects $(x_1, \ldots, x_m)$, embed them by some embedder $\phi$, then compute the similarity matrix $R = \text{Softmax}(A), A = {\left[\langle\phi(x_i), \phi(x_j)\rangle\right]}_{ij}$. In this form, CoRelNet models relations as necessarily symmetric. It can be modified to support asymmetric relations via the natural modification $A = {\left[\langle W_1 \phi(x_i), W_2 \phi(x_j)\rangle\right]}_{ij}$, where $W_1, W_2$ are trainable matrices. In~\citep{kerg2022neural} the authors argue that symmetry is an important inductive bias. The following simple experiment demonstrates that, while symmetry may be a useful inductive bias on relational tasks where the underlying relation is symmetric, the ability to model asymmetric relations is necessary for more general tasks.

% Another limitation is that it can only model single-dimensional relations---for each pair of objects $(i,j)$, their modeled relation is a single-dimensional scalar $R_{ij}$. The Abstractor is able to model a significantly larger class of relations. In particular, it is able to model asymmetric and multi-dimensional relations through the $\text{MultiHeadRelation}$ operation. This is demonstrated by the following simple experiment.

We generate $N = 32$ ``random objects'' represented by iid Gaussian vectors, $o_i \overset{iid}{\sim} \mathcal{N}(0,
I_d) \in \mathbb{R}^d$, and associate an order relation to them $o_1 \prec o_2 \prec \cdots \prec o_N$. Note that $\prec$ is \textit{not symmetric}. Of the $N^2 = 1024$ possible pairs $(o_i, o_j)$, 15\% are held out as a validation set (for early stopping) and 35\% as a test set. We evaluate learning curves by training on the remaining 50\% and computing accuracy on the test set (10 trials for each training set size). Note that under this set up, we are evaluating the models on pairs they have never seen. Thus, the models will need to generalize based on the transitivity of the $\prec$ relation.

We compare three models: an Abstractor, standard (symmetric) CoRelNet, and asymmetric CoRelNet. We observe that standard symmetric CoRelNet is completely unable to learn the task, whereas the Abstractor and asymmetric CoRelNet learn the transitive $\prec$ relation~(\Cref{fig:exp_order_relation}).~\citep{kerg2022neural} finds symmetry to be an important inductive bias for the relational tasks they consider (which are based on a simple same/different underlying relation), whereas we find that the ability to model asymmetric relations is necessary for more general tasks. This can be explained in terms of the relational bottleneck. In a relational task, there exists a sufficient statistic which is relational. The relational bottleneck restricts the space of learnable representations to be the space of relational features, thus making the search for a good representation easier and more sample efficient. In a relational task in which there exists a sufficient statistic involving a symmetric relation (as is the case with same/different tasks), we can further restrict the search space to be over symmetric relational representations, which should make learning a good representation even more sample efficient. Since the experiments \citep{kerg2022neural} considers are indeed symmetric, symmetry was a useful inductive bias. However, some relations are more complex and may be asymmetric---an example is order relations. Symmetric inner products don't have the representational capacity to model such relations. But asymmetric inner products with different learned left and right encoders can model such relations.

\subsubsection{SET: modeling multi-dimensional relations}\label{sssec:exp_set}

The $\prec$ relation is a one-dimensional relation. Similarly, the underlying relations in the experiments considered in~\citep{kerg2022neural} are also one-dimensional (same/different). In the next experiment, we explore a discriminative relational tasks which relies on a multi-dimensional relation. The task we consider is SET. 

\begin{wrapfigure}{R}{0.25\textwidth}
	\vskip-5pt
	\begin{tabular}{c}
		\includegraphics[width=.25\textwidth]{figures/set_example}\\[-5pt]
	\end{tabular}
	\caption{\footnotesize The SET game}
\end{wrapfigure}

SET is a relatively straightforward but challenging cognitive task that engages reasoning faculties in a deliberative, attentionally directed manner, requiring several levels of abstraction over sensory information. Players are presented with a sequence of cards, each of which contains figures that vary along four dimensions (color, number, pattern, and shape) and they must find triplets of cards which obey a deceptively simple rule: along each dimension, cards in a SET must either have the same value or three unique values. For example, in the figure to the right, the cards with two solid blue/purple diamonds, two striped blue squiggles, and two open blue oblongs form a SET: same color, same number, different patterns, different shapes.

In this experiment, the task is, given a triplet of card images, to determine whether they form a SET or not. A CNN classifier is trained on the card images to predict the four attributes. An intermediate layer is used as an embedder for all relational models. We compare an Abstractor model to CorelNet. The shared architecture is $\texttt{CNN} \to \{\texttt{Abstractor} \text{ or } \texttt{CorelNet}\} \to \texttt{Flatten} \to \texttt{Dense}$. We report learning curves in~\Cref{fig:exp_set_classification} (10 trials per training set size). We find that the Abstractor model significantly out-performs CoRelNet. We attribute this to its ability to model multi-dimensional relations. In this task, there exists four different relations (one for each attribute) which are needed to determine whether a triple of cards forms a set. CoRelNet would need to squeeze all of this information into a single-dimensional scaler whereas the Abstractor can model each relation separately. We hypothesize that the ability to model relations as multi-dimensional is also the reason that the Abstractor can learn the order relation better than asymmetric CoRelNet---even though the underlying relation is one-dimensional, having a multi-dimensional representation enables greater robustness and multiple avenues towards a good solution during optimization.

\begin{figure}[t]
    % \vskip-.2in
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        %\hskip-.35in
        \includegraphics[width=\textwidth]{figures/experiments/pairwise_order_learning_curves.pdf}
        % \vskip-5pt
        \caption{The $\prec$ relation can be learned with asymmetric but not symmetric inner products.}\label{fig:exp_order_relation}
    \end{subfigure} 
    \hskip10pt
    % \captionsetup[subfigure]{oneside,margin={-.3in,0in}}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        % \vskip10pt
        % \hskip-.6in
        \includegraphics[width=\textwidth]{figures/experiments/set_classification.pdf}
        % \vskip-5pt
        \caption{The Abstractor's ability to model multi-dimensional relations enables it to solve SET.}\label{fig:exp_set_classification}
    \end{subfigure}
    \caption{Experiments on discriminative relational tasks and comparison to CoRelNet.}
\end{figure}


==> experiments_object_sorting_longer.tex <==
\subsection{Object-sorting: purely relational sequence-to-sequence tasks}\label{ssec:experiments_object_sorting}

In the following set of experiments, we consider sequence-to-sequence tasks which are purely relational, and compare an Abstractor-supported model to a plain Transformer. We consider the task of \textit{sorting} sequences of randomly permuted random objects. These experiments are ``purely relational'' in the sense that there exists a relation (order) which is a sufficient statistic for solving the task---the features of individual objects beyond this relation are extraneous. This is a more controlled setting which tests the hypothesis that the inductive biases of the Abstractor indeed confer benefits in modeling relations. We consider the more ``realistic'' setting of partially-relational tasks in the next section. The experiments in the present section demonstrate that the Abstractor enables a dramatic improvement in sample-efficiency on sequence-to-sequence relational tasks.
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \hskip-.35in\includegraphics[width=\textwidth]{figures/experiments/random_object_sorting.pdf}
        \vskip-5pt
        \caption{Learning curves on sorting sequences of random objects. The abstractor is dramatically more sample-efficient.}\label{fig:exp_object_sorting}
    \end{subfigure}\hspace{\fill}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \hskip-.6in\includegraphics[width=\textwidth]{figures/experiments/random_object_sorting_generalization.pdf}
        \vskip-5pt
        \caption{Learning curves with and without pre-training on a similar sorting task. The Abstractor benefits from pre-training.}\label{fig:exp_object_sorting_generalization}
    \end{subfigure}
    % \bigskip
    \caption{Experiments on purely relational sequence-to-sequence tasks.}\label{fig:experiments}
    \vskip-.10in
\end{figure}

\subsubsection{Superior sample-efficiency on relational seq2seq tasks compared to standard transformers}\label{sssec:exp_object_sorting_sample_efficiency}

We generate random objects in the following way. First, we generate two sets of random attributes $\mathcal{A} = \{a_1, a_2, a_3, a_4\}$, $a_i \overset{iid}{\sim} \mathcal{N}(0, I) \in \mathbb{R}^{4}$ and $\mathcal{B} = \{b_1, \ldots, b_{12}\}$, $b_i \overset{iid}{\sim} \mathcal{N}(0, I) \in \mathbb{R}^{8}$. To each set of attributes, we associate the strict ordering relation $a_1 \prec a_2 \prec a_3 \prec a_4$ and $b_1 \prec b_2 \prec \cdots \prec b_{12}$, respectively. Our random objects are formed by the Cartesian product of these two attributes $\mathcal{O} = \mathcal{A} \times \mathcal{B}$, yielding $N = 4 \times 12 = 48$ objects (i.e.: each object in $\mathcal{O}$ is a vector in $\mathbb{R}^{4+8}$ formed by a concatenation of one attribute value in $\mathcal{A}$ and one in $\mathcal{B}$). Then, we associate with $\mathcal{O}$ the strict ordering relation corresponding to the order relation of $\mathcal{A}$ as the primary key and the order relation of $\mathcal{B}$ as the secondary key. i.e.: $(a_i, b_j) \prec (a_k, b_l)$ if $a_i \prec a_k$ or if $a_i = a_k$ and $b_j \prec b_l$.

Given a set of objects in $\mathcal{O}$, the task is to sort it according to $\prec$. More precisely, the input sequences are randomly permuted sequences of $10$ objects in $\mathcal{O}$ and the target sequences are the indices of the object sequences in sorted order (i.e., the `argsort'). The training data are sampled uniformly from the set of length-10 sequences in $\mathcal{O}$. We also generate a non-overlapping validation dataset (used during training for early stopping) and a testing dataset (used during evaluation).

We evaluate learning curves on an Abstractor, a Transformer, and an ``Ablation'' model (10 trials for each training set size). The Abstractor uses the architecture $\texttt{Encoder} \to \texttt{Abstractor} \to \texttt{Decoder}$ (architecture (b) in~\Cref{fig:abstractor_architectures}). The Encoder-to-Abstractor interface uses relational cross-attention and the Abstractor-to-Decoder interface uses standard cross-attention. The Ablation Model aims to test the effects of the relational cross-attention in the Abstractor model---it is architecturally identical to the Abstractor model with the crucial exception that the Encoder-to-Abstractor interface instead uses standard cross-attention. The hyperparameters of the models are chosen so that the parameter counts are similar. % TODO: add details here? or in supplement?
We find that the Abstractor is dramatically more sample-efficient than the Transformer and the Ablation model~(\Cref{fig:exp_object_sorting}).

\subsubsection{Ability to generalize to similar tasks}\label{sssec:exp_object_sorting_generalization}

Continuing with the object-sorting task and the dataset generated as described above, we test the Abstractor's ability to generalize from similar relational tasks through pre-training. The main task uses the same dataset described above. The pre-training task involves the same object set $\mathcal{O}$ but the order relation is changed. The ordering in attribute $\mathcal{A}$ is randomly permuted, while the ordering in attribute $\mathcal{B}$ is kept the same. A strict ordering relation $\prec$ on $\mathcal{O}$ is obtained in the same way---using the order in $\mathcal{A}$ as the primary key and the order in $\mathcal{B}$ as the secondary key.

The Abstractor model here uses the architecture $\texttt{Abstractor} \to \texttt{Decoder}$ (i.e.: no Transformer
encoder), and the transformer is the same as the previous section. We pre-train both models on the pre-training task
and then, using those learned weights for initialization, evaluate learning curves on the original task. Since the
Transformer requires more training samples to learn the object-sorting task, we use a pre-training set size of $3,000$, chosen based on the results of the previous subsection so that it is large enough for the Transformer to learn the pre-training task. This experiment assesses the models' ability to generalize relations learned on one task to a new task.~\Cref{fig:exp_object_sorting_generalization} shows the learning curves for each model with and without pre-training. We observe that when the Abstractor is pre-trained, its learning curve on the object-sorting task is significantly accelerated. The transformer does not benefit from pre-training.


==> figures/experiments/math_tfm_metrics_table.tex <==
\begin{tabular}{llrr}
\toprule
                    &                       &  tf acc &  tf acc (val) \\
task & model &         &               \\
\midrule
algebra\_\_linear\_1d & transformer &   0.792 &         0.733 \\
                    & transformer+ &   0.776 &         0.603 \\
                    & relational\_abstractor &   0.834 &         0.791 \\
algebra\_\_sequence\_next\_term & transformer &   0.889 &         0.881 \\
                    & transformer+ &   0.922 &         0.918 \\
                    & relational\_abstractor &   0.916 &         0.922 \\
calculus\_\_differentiate & transformer &   0.996 &         0.998 \\
                    & transformer+ &   0.998 &         0.998 \\
                    & relational\_abstractor &   0.999 &         1.000 \\
polynomials\_\_add & transformer &   0.851 &         0.841 \\
                    & transformer+ &   0.860 &         0.851 \\
                    & relational\_abstractor &   0.869 &         0.863 \\
polynomials\_\_coefficient\_named & transformer &   0.587 &         0.549 \\
                    & transformer+ &   0.603 &         0.564 \\
                    & relational\_abstractor &   0.630 &         0.599 \\
polynomials\_\_expand & transformer &   0.804 &         0.774 \\
                    & transformer+ &   0.817 &         0.785 \\
                    & relational\_abstractor &   0.847 &         0.821 \\
\bottomrule
\end{tabular}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related_work.tex <==
\subsection{Related Work}\label{ssec:related_work}
A growing body of literature is focused on developing machine learning architectures with explicit relational reasoning capabilities. An early example is the Relation Network proposed in~\citep{santoro1}, which proposes modeling pairwise relations by applying an MLP to the concatenation of object representations and aggregating the outputs by a simple summation.~\citep{shanahanExplicitlyRelationalNeural} proposes the PrediNet architecture which aims to learn representations of relations in a manner inspired by predicate logic. The ESBN model proposed in~\citep{esbn} is a memory-augmented LSTM network, inspired by ideas from cognitive science, which aims to factor representations into `sensory' and `relational'. In this sense, it is similar in spirit to the present work. Another architecture which is similar in spirit is the CoRelNet architecture proposed in~\citep{kerg2022neural}, which reduces relational learning to modeling a similarity matrix.

The Transformer~\citep{vaswani2017attention} is a common baseline which is compared against in this literature. It is shown in these works that explicitly relational architectures outperform the Transformer, sometimes by large margins, on several synthetic discriminative relational tasks~\citep{shanahanExplicitlyRelationalNeural,esbn,kerg2022neural}. In this work, we offer an explanation, arguing that while the Transformer architecture is versatile enough to learn such relational tasks given enough data, it does not support relational reasoning explicitly. The Abstractor module extends the Transformer framework by learning representations of relations which are disentangled from extraneous object-level features. Our experiments first validate that the Abstractor, on its own, achieves the same sample-efficiency gains of other relational architectures on discriminative relational task. We then evaluate whether the Abstractor can augment a Transformer to improve relational reasoning by evaluating on synthetic \textit{sequence-to-sequence} relational tasks, which has so far been unexplored in the literature on explicitly relational architectures. Finally, we evaluate an Abstractor-based architecture on a more realistic mathematical problem-solving task to evaluate the potential of the idea on more general tasks.
